Plane Geometry Problem Solving with Multi-modal Reasoning: A Survey

Plane geometry problem solving (PGPS) has recently gained significant attention as a benchmark to assess the multi-modal reasoning capabilities of large vision-language models. Despite the growing interest in PGPS, the research community still lacks a comprehensive overview that systematically synthesizes recent work in PGPS. To fill this gap, we present a survey of existing PGPS studies. We first categorize PGPS methods into an encoder-decoder framework and summarize the corresponding output formats used by their encoders and decoders. Subsequently, we classify and analyze these encoders and decoders according to their architectural designs. Finally, we outline major challenges and promising directions for future research. In particular, we discuss the hallucination issues arising during the encoding phase within encoder-decoder architectures, as well as the problem of data leakage in current PGPS benchmarks.

==> appendices/PGPS_datasets.tex <==
\section{PGPS Datasets}

\subsection{Summary of PGPS datasets}

\input{tables/pgps_lvlm_datasets}

We summarize the PGPS datasets and benchmarks in the perspective of input-output format and the collection method at \cref{tab:dataset_overview}.


==> figures/pgps_datasets.tex <==
% \begin{table*}[t]
%     \centering
%     \renewcommand{\arraystretch}{1.15}
%     \begin{tabular}{p{0.30\linewidth} p{0.23\linewidth} p{0.44\linewidth}}
%         \toprule
%         \textbf{Input–output representation} & \textbf{Collection method} & \textbf{Datasets} \\
%         \midrule
%         \multirow{2}{*}{Benchmark only} 
%             & Human annotation & GeoShader, MathVerse, MathVista, MMMU, MATH-V, DynaMath, GeoSense, VCBench, PolyMath \\
%             & Synthetic annotation & GeoTrust,\;GeomVerse,\;VisOnlyQA \\
%         \midrule
%         Diagram $\rightarrow$ formal-language description 
%             & Human annotation & GEOS, GEOS++, GEOS-OS, Geometry3K, PGDP5K, PGPS9K, formalgeo7k \\
%         \midrule
%         Formal-language description $\rightarrow$ theorem sequences 
%             & Human annotation & GEOS++, GEOS-OS, Geometry3K, formalgeo7k \\
%         \midrule
%         Problem $\rightarrow$ logic program 
%             & Human annotation & GeoQA, GeoQA+, PGPS9K, UniGeo \\
%         \midrule
%         \multirow{2}{*}{Problem $\rightarrow$ natural-language description} 
%             & L(V)LM-assisted annotation & G-LLaVA, MATH-LLaVA, GPSM4K, MAVIS \\
%             & Synthetic annotation & MAVIS \\
%         \bottomrule
%     \end{tabular}
%     \caption{Datasets grouped by their input–output representation and collection method.}
%     \label{tab:dataset_overview}
% \end{table*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=.9\linewidth]{figures/images/pgps_datasets.pdf}
    % \begin{subfigure}[t]{\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/images/pgps_datasets_diagram.pdf}
    %     \caption{Diagram-only and relation set input PGPS datasets}
    % \end{subfigure}
    % \begin{subfigure}[t]{\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/images/pgps_datasets_diagram_text.pdf}
    %     \caption{Diagram and text input PGPS datasets}
    % \end{subfigure}
    \caption{Examples of problem-solution format of PGPS problems. Several PGPS datasets and benchmarks represent plane geometry problems differently, such as: i) converting diagrams to formal-language descriptions, ii) translating formal-language descriptions into sequences of theorems, iii) mapping diagram-text pairs to logic programs, or iv) generating natural-language descriptions from diagrams and text.}
    \label{fig:pgps_datasets}
\end{figure*}

==> sections/2.related_work.tex <==
\section{Related Work}



==> tables/datasets.tex <==

\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{p{0.30\linewidth} p{0.23\linewidth} p{0.44\linewidth}}
        \toprule
        \textbf{Input–output representation} & \textbf{Collection method} & \textbf{Datasets} \\
        \midrule
        \multirow{2}{*}{Benchmark only} 
            & Human annotation & GeoShader, MathVerse, MathVista, MMMU, MATH-V, DynaMath, GeoSense, VCBench, PolyMath \\
            & Synthetic annotation & GeoTrust,\;GeomVerse,\;VisOnlyQA \\
        \midrule
        Diagram $\rightarrow$ formal-language description 
            & Human annotation & GEOS, GEOS++, GEOS-OS, Geometry3K, PGDP5K, PGPS9K, formalgeo7k \\
        \midrule
        Formal-language description $\rightarrow$ theorem sequences 
            & Human annotation & GEOS++, GEOS-OS, Geometry3K, formalgeo7k \\
        \midrule
        Problem $\rightarrow$ logic program 
            & Human annotation & GeoQA, GeoQA+, PGPS9K, UniGeo \\
        \midrule
        \multirow{2}{*}{Problem $\rightarrow$ natural-language description} 
            & L(V)LM-assisted annotation & G-LLaVA, MATH-LLaVA, GPSM4K, MAVIS \\
            & Synthetic annotation & MAVIS \\
        \bottomrule
    \end{tabular}
    \caption{Datasets grouped by their input–output representation and collection method.}
    \label{tab:dataset_overview}
\end{table*}

% \begin{table*}[b!]
%     \centering
%     \caption{Geometric Benchmarks for Supervised Models}
%     \label{tab:my_label}
%     \begin{tabular}{l c r c c c}
%         \toprule
%         Dataset & Problem type & Quantity & \# sources & OCR & Difficulty\\
%         \midrule
%         ShadedArea \\
%         G-Aligner~\cite{g-aligner} & GPD, GPA & 100 & 4 & $\bigcirc$\\
%         GeoS~\cite{seo2015solving} & GPS & 119 & 1 & $\bigcirc$\\
%         GeoS++~\cite{geos-plus} & GPS & 906 & 5 & $\bigcirc$\\
%         GeoQA~\cite{geoqa} & GPS & 754 & 2 & $\times$\\
%         UniGeo~\cite{unigeo} & GTP & 1,447 & 1 & $\times$\\
%         Geometry3K~\cite{lu2021intergps} & GPS & 601 & 2& $\times$\\
%         GeometryQA \\
%         GeoRE \\
%         GeoEval \\
%         PGDP5K~\cite{zhang2022pgdpnet} & GPD, GRD & 1,000 & 4 & $\bigcirc$\\
%         PGPS9K~\cite{pgps} & GPS & 1,000 & 2 & $\times$\\
%         formalgeo7k \\
%         \bottomrule
%     \end{tabular}
% \end{table*}

% \begin{table*}[b!]
%     \centering
%     \caption{Benchmarks 2}
%     \label{tab:my_label2}
%     \begin{tabular}{l l c c c c}
%         \toprule
%         Dataset & Sources & Reasoning & Difficulty & Perception & Robustness \\
%         \midrule
%         MathVista~\cite{mathvista} & Geometry3K, GeoQA+, UniGeo, GeoS & $\bigcirc$& $\times$ & $\times$ & $\times$ \\
%         MMMU~\cite{mmmu} & Unknown & $\bigcirc$& $\times$ & $\times$ & $\times$ \\
%         Math-V~\cite{math-v} & 19 competitions & $\bigcirc$& $\times$ & $\times$ & $\times$ \\
%         GeomVerse~\cite{geomverse} & Synthetic & $\bigcirc$& $\bigcirc$ & $\times$ & $\times$ \\
%         MathVerse~\cite{mathverse} & Geometry3K, GeoQA, GeoS, three manual sites & $\bigcirc$& $\times$ & $\bigcirc$ & $\times$\\
%         DynaMath~\cite{dynamath} & MathVista & $\bigcirc$& $\times$ & $\times$ & $\bigcirc$ \\
%         CogAlign~\cite{cogalign} & Synthetic & $\times$& $\times$ & $\bigcirc$ & $\times$ \\
%         VisOnlyQA~\cite{visonlyqa} & Synthetic & $\times$& $\times$ & $\bigcirc$ & $\times$ \\
%         \bottomrule
%     \end{tabular}
% \end{table*}



==> tables/pgps_lvlm_datasets.tex <==
\begin{table*}[t]
    \centering
    % \renewcommand{\arraystretch}{1.15}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llp{0.4\linewidth}}
        \toprule
        \textbf{Input–output format} & \textbf{Collection method} & \textbf{Datasets and benchmarks} \\
        \midrule
        Problem to scalar value or choice & Human annotation & GEOS~\citep{geos}, GeoShader~\citep{GeoShader}, Geometry3K~\citep{intergps}, GeoQA~\citep{geoqa}, GeoQA+~\citep{geoqa+}, PGPS9K~\citep{pgps9k}, formalgeo7k~\citep{formalgeo7k}, MathVerse~\citep{mathverse}, MathVista~\citep{mathvista}, MMMU~\citep{mmmu}, MATH-V~\citep{Math-Vision}, DynaMath~\citep{dynamath}, GeoSense~\citep{geosense}, VCBench~\citep{vcbench}, PolyMath~\citep{polymath} \\
        & Synthetic annotation & GeoTrust~\citep{TrustGeoGen}, GeomVerse~\citep{geomverse}, VisOnlyQA~\citep{visonlyqa} \\
        % \multirow{2}{*}{Benchmark only} 
        %     & Human annotation & GeoShader, MathVerse, MathVista, MMMU, MATH-V, DynaMath, GeoSense, VCBench, PolyMath \\
        %     & Synthetic annotation & GeoTrust,\;GeomVerse,\;VisOnlyQA \\
        \midrule
        Diagram to formal-language description 
            & Human annotation & GEOS~\citep{geos}, GEOS++~\citep{geos++}, GEOS-OS~\citep{GEOS-OS}, Geometry3K~\citep{intergps}, PGDP5K~\citep{pgdp5k}, PGPS9K~\citep{pgps9k}, formalgeo7k~\citep{formalgeo7k} \\
        \midrule
        Formal-language description to theorem sequences 
            & Human annotation & GEOS++~\citep{geos++}, GEOS-OS~\citep{GEOS-OS}, Geometry3K~\citep{intergps}, formalgeo7k~\citep{formalgeo7k} \\
        \midrule
        Problem to logic program 
            & Human annotation & GeoQA~\citep{geoqa}, GeoQA+~\citep{geoqa+}, PGPS9K~\citep{pgps9k}, UniGeo~\citep{unigeo} \\
        \midrule
        Problem to natural-language description & L(V)LM-assisted annotation & G-LLaVA~\citep{G-LLaVA}, MATH-LLaVA~\citep{math-llava}, GPSM4K~\citep{GPSM4K}, MAVIS~\citep{mavis} \\
        & Synthetic annotation & MAVIS~\citep{mavis}, GeoDANO~\citep{GeoDANO} \\
        % \multirow{2}{*}{Problem $\rightarrow$ natural-language description} 
        %     & L(V)LM-assisted annotation & G-LLaVA, MATH-LLaVA, GPSM4K, MAVIS \\
        %     & Synthetic annotation & MAVIS \\
        \bottomrule
    \end{tabular}
    }
    \caption{Summary of input-output formats, collection methods, and associated PGPS datasets and benchmarks. We categorize the existing PGPS datasets and benchmarks based on the input-output format and the collection strategy.}
    \label{tab:dataset_overview}
\end{table*}

% \begin{table*}[t!]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lp{8cm}}
% \toprule
% \textbf{Datasets} & \textbf{Sources of diagrams} \\
% \midrule
% G\textendash{}LLaVA~\citep{G-LLaVA} & GeoQA$+$, Geometry3K \\
% MAVIS~\citep{mavis} & Synthetic; Geometry3K, GeoQA$+$; 4{,}000 manually collected problems \\
% Math\textendash{}LLaVA~\citep{math-llava} & GEOS, GeoQA$+$, Geometry3K, UniGeo \\
% CogAlign~\citep{CogAlign} & Synthetic \\
% VisOnlyQA~\citep{visonlyqa} & Synthetic \\
% GPSM4K~\citep{GPSM4K} & \\
% \midrule
% \textbf{Benchmarks} & \textbf{Sources of problems} \\
% \midrule
% MMMU~\citep{mmmu}          & Unknown \\
% Math\textendash V~\citep{Math-Vision}      & 19 competitions (e.g., AMC 8, 10, 12) \\
% MathVista~\citep{mathvista}      & GEOS, GeoQA$+$, Geometry3K, UniGeo \\
% MathVerse~\citep{mathverse}      & GeoQA, GEOS, Geometry3K; plus 370 manually collected from internet \\
% GeomVerse~\citep{geomverse}      & Synthetic (algorithmically generated) \\
% DynaMath~\citep{dynamath}       & Seeded from Math\textendash V \\
% VisOnlyQA~\citep{visonlyqa}      & Synthetic \\
% MM\textendash MATH~\citep{mm-math}      & 21st Century Education Network \\
% GeoEval~\citep{geoeval}        & Geometry3K, PGPS9K, UniGeo, GeoQA$+$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}
